Blocked or Broken? Automatically Detecting When Privacy Interventions Break Websites

A core problem in the development and maintenance of crowd-sourced filter lists is that their maintainers cannot confidently predict whether (and where) a new filter list rule will break websites. This is a result of enormity of the Web, which prevents filter list authors from broadly understanding the impact of a new blocking rule before they ship it to millions of users. The inability of filter list authors to evaluate the Web compatibility impact of a new rule before shipping it severely reduces the benefits of filter-list-based content blocking: filter lists are both overly-conservative (i.e. rules are tailored narrowly to reduce the risk of breaking things) and error-prone (i.e. blocking tools still break large numbers of sites). To scale to the size and scope of the Web, filter list authors need an automated system to detect when a new filter rule breaks websites, before that breakage has a chance to make it to end users. In this work, we design and implement the first automated system for predicting when a filter list rule breaks a website. We build a classifier, trained on a dataset generated by a combination of compatibility data from the EasyList project and novel browser instrumentation, and find it is accurate to practical levels (AUC 0.88). Our open source system requires no human interaction when assessing the compatibility risk of a proposed privacy intervention. We also present the 40 page behaviors that most predict breakage in observed websites.

==> Makefile <==
extensions_to_clean := out aux log bbl blg fls fdb_latexmk glg gls lof glo glsdefs lot toc dvi ist acn acr synctex.gz alg xdy

all: paper

clean:
	@if [[ -f paper.pdf ]]; then \
		rm paper.pdf;\
	fi;
	@for extension in $(extensions_to_clean); do \
		find . -type f -name "*.$$extension" -delete;\
	done;
	@rm -f diff.*

paper:
	latexmk -bibtex -pdf paper
	pdflatex -bibtex -interaction=batchmode paper

diff:
	latexmk -bibtex -pdf diff
	pdflatex -bibtex -interaction=batchmode diff


==> figures/behaviour-feature-imp.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{graphics/behaviour-feature-group-imp.pdf}
    \caption{\ROCAUC{} curves averaged over \NumOuterFolds{} folds with hyper-parameter tuning to evaluate the practical utility of the classifier.}
    \label{figure:behaviour_feature_imp}
\end{figure}

==> paper_pets.tex <==
% \documentclass[USenglish,oneside,twocolumn]{article}

% \usepackage[utf8]{inputenc}
% \usepackage[big]{dgruyter_NEW}
% \makeatletter
% \p@=1pt
% \makeatother

% \usepackage{xspace}
% \usepackage{multirow}


% \usepackage{xargs}
% \usepackage[pdftex,dvipsnames]{xcolor}
% \usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
% \newcommandx{\xxx}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}

% \usepackage{listings}
% \usepackage{./lstlinebgrd}

% \input{includes/abbr}
% \input{includes/colors}
% \input{includes/commands}
% \input{includes/data}
% \input{includes/syntax}

% \cclogo{\includegraphics{graphics/by-nc-nd.pdf}}

% \usepackage{tikz}
% \usetikzlibrary{arrows.meta}
% \usetikzlibrary{positioning}
% \tikzset{%
%   >={Latex[width=2mm,length=2mm]},
%         base/.style = {rectangle, rounded corners, draw=black,
%                           minimum width=1cm, minimum height=1cm,
%                           align=center, font=\sffamily},
%         parser/.style = {fill=red!10},
%         dom/.style = {fill=blue!10},
%         resource/.style = {fill=yellow!10},
%         sect/.style = {rectangle, draw=black,
%                   minimum width=8.2cm, minimum height=1cm,
%                   align=center, font=\footnotesize\sffamily, fill=yellow!10},
%         user/.style = {rectangle, draw=white,
%                       align=center, font=\footnotesize\sffamily},
%         result/.style = {rectangle, rounded corners, draw=black,
%                           minimum width=1cm, minimum height=1cm,
%                           align=center, font=\footnotesize\sffamily, fill=pink!20},
% }

% \begin{document}

% \title{Blocked or Broken? Automatically Detecting When Privacy Interventions Break Websites}
% \runningtitle{Did It Break?}

% \input{sections/0_abstract}

% \keywords{content blocking, Web compatibility}
% \journalname{Proceedings on Privacy Enhancing Technologies}
% \startpage{1}
% %\received{..}
% %\revised{..}
% %\accepted{..}
% \journalyear{..}
% \journalvolume{..}
% \journalissue{..}

% \maketitle

% \input{sections/1_intro}
% \input{sections/2_motivation}
% \input{sections/3_dataset}
% \input{sections/4_classifier}
% \input{sections/5_results}
% \input{sections/6_discussion}
% \input{sections/7_related_work}
% \input{sections/8_conclusion}

% \bibliographystyle{IEEEtran}
% \bibliography{paper}

% \end{document}


==> unused-bits/2_motivation.tex <==

This section provides a representative example of why it is difficult
for filter list authors to reason about the compatibility-impact
of new rules \emph{before those rules are shipped}.
We then use this example to motivate why an automated system
to predict whether a filter list rule would break a website
would be helpful to the maintenance and development of
crowd sourced filter lists.


\subsection{Filter List Capabilities}
\label{sec:motiviation:capabilties}
We first summarize how common filter lists work, and what options
filter lists maintainers have when authoring a new filter list rule.
There are many different filter list formats, each providing slightly
different options to filter list authors\footnote{For example,
AdBlock Plus, uBlock Origin, AdGuard, and Brave all support slightly different
implementations of, and extensions to, whats sometimes called ``ABP filter syntax''.}
For the purposes of this work though, we only consider features common
to all of the most popular  filter list formats.

Filter list authors can make rules very general (\IE{} ``block all requests
for URL X, across the entire \Web{}``), very specific (\IE{} ``block requests for
URL X, but only when loaded on website Y; load requests to X elsewhere''),
or anything in between. Filter list authors can narrow
the application of a filter list rule in other ways too (\EG{} ``block
requests for URL X only, when its being fetched as an image``). Finally,
filter list authors can further narrow the application of a rule by
creating ``exception'' rules, which denote ``always load requests
for URL X, even if another rule exists instructing you to block
URL X.''


\subsection{Guessing Optimal Blocking Granularity}
\label{sec:motivation:optimal}

Though filter list authors have many ways of controlling how
widely or narrowly a rule will be applied, they face serious
difficulties when deciding how to use those capabilities.
To see why, consider the following representative example.

Assume that a filter list author identifies a new privacy harming
\JS{} resource being loaded across the \Web{}. This hypothetical
script is popular, and loaded on a significant percentage
of the \Web{}; enough of the \Web{} that it its not practical
for the filter list authors to manually evaluate every page
the script is loaded on.

The filter list author would like to add a rule to block the resource 
as broadly as possible, \emph{except} when blocking the resource would
break a \Web{} page. If the filter list author makes the rule too
general (say, by applying the rule to the entire Web), the author
risks breaking pages for users. On the
other hand, if the author makes the rule to specific (say, by only
applying the rule to websites the author has visited themselves), the
author allows privacy harm, including potentially privacy-harm that could be
prevented with no downside (\IE{} websites where the script could be blocked
without breaking the page).


\subsection{Motivation Conclusion}
\label{sec:motivation:conclusion}

The root, what makes figuring out the optimal granularity of a filter list
rule difficult is simple: the \Web{} is enormous, evaluating the
compatibility impact of a filter list rule is to date a manual process, and
filter list author time is limited. An automated technique to determine
if, and which, websites will break if a filter list rule is added would
maintain and expand the benefits of filter lists. Filter list authors
could deploy such automated tools to a far greater portion of the \Web{}
than they can manually evaluate, allowing filter list authors to better
understand the compatibility-impact of a rule \emph{before shipping the rule
to users}.
Filter list authors
could then be both more aggressive in blocking requests (knowing which sites
a rule breaks would remove the need to be conservative when adding new rules),
and lessen the need for filter list users to disable blocking tools to use
broken sites.

The rest of this work presents the design of such a system, a fully automated
system for evaluating whether a filter list rule would break a given website.

==> unused-bits/6_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

We next provide some discussion of how our system could be deployed, extended
and improved by future work. We first discuss practical deployment scenarios
for our compatibility classifier, and how our system could be used by
filter list authors to improve the compatibility and coverage
of crowd sourced filter lists. Next, we discuss how our approach could
be extend to other, non-filter list privacy interventions, and the potential
difficulties in doing so. Last, we discuss some of the limitations and weaknesses
in our approach, and how they could be addressed by future work.

\subsection{Deployment Strategies}
\label{suc:discussion:deployment}

We expect the automated compatibility classifier described in this work will
help filter list authors improve the compatibility and coverage of crowd-sourced filter lists.
Replacing the current system of for handling filter-list compatibility (\IE{} best-effort expert intuition
and manual evaluation) with a fully automated approach should allow for more sites to be
checked for compatibility issues, far more often.

However, figuring out \emph{how} to use our system to improve filter list development is not
as simple a problem as it might at first seem. First, the size and churn of the \Web{}, coupled with the ever growing
size of filter lists\cite{snyder2020filters} makes a straight forward ``measure everything'' approach infeasible.
Second, filter lists are maintained by a mixture of hobbyists, activists, and (comparatively) small 
privacy-focused companies and organizations; practical deployments likely will not have access to
\Web{} scale measurement resources. And third, while our classifier is accurate (to useful
levels, see Section \ref{sec:evaluation_and_results:utility}), its not perfect; practical deployments
should admit and compensate for the significant-but-imperfect accuracy of the classifier, not build from
the assumption that its an perfect oracle.

To that end, we present three deployment strategies for our classifier. We intend these strategies
to compose together, and to most-benefit users that are under-served by existing filter lists.


\subsubsection{Assisting Existing Filter List Curators}
First, we propose using our classifier to assist, instead of replace, existing filter
list developers. In this scenario, the goal of the classifier would be to reduce
the number of sites that needed a manual compatibility evaluation each time a 
new rule was proposed.  The classifier would serve as a ``force-multipler'' for
human evaluators then, allowing the same number of filter list authors to anticipate
the compatibility risks of a larger number of
then allow the same number
of filter list authors to 

Our classifier could be tuned to, say, prefer recall over precision. 




\subsection{Applicability to Other Privacy Interventions}

\subsection{Limitations and Future Work}

==> unused-bits/feature-imp-table.tex <==
\begin{table}
  \begin{center}
    \small
      \begin{tabular}{lll}
          \toprule
          Features & AUC Loss & Rank \\
          \midrule
          General Features & \\
          \midrule
           No. of Unique Source Node Types & 0.0018 & 11 \\
           No. of Unique Edge Types & 0.0006 & 22 \\
           No. of Unique Edge Types & 0.0002 & 35 \\
          \midrule
          Features Targeting Page Structure & \\
          \midrule
           No. of Source Nodes of Type DOM Root & 0.0037 & 3 \\
           No. of Source Nodes of Type Parser & 0.0022 & 6 \\
           No. of Target Nodes of Type DOM Root & 0.0016 & 13 \\
           No. of Source Nodes of Type Frame Owner & 0.0008 & 19 \\
           No. of WebGL Web API Calls & 0.0007 & 20 \\
           No. of Source Nodes of Type HTML Element & 0.0002 & 33 \\
           No. of Source Nodes of Type Frame Owner & 0.0002 & 36 \\
           No. of HTML Elements Created & 0.0001 & 40 \\
          \midrule
          Features Targeting \JS{} Behaviors & \\
          \midrule
           No. of Navigator Web API Calls & 0.0030 & 4 \\
           No. of Edges of Type Execute & 0.0025 & 5 \\
           No. of Session Storage Delete Storage Calls & 0.0022 & 8 \\
           No. of Cookie Jar Set Storage Calls & 0.0021 & 9 \\
           No. of Source Nodes of Type Local Storage & 0.0019 & 10 \\
           No. of Edges of Type Execute & 0.0013 & 14 \\
           No. of Cookie Jar Read Storage Calls & 0.0012 & 15 \\
           No. of Source Nodes of Type Cookie Jar & 0.0011 & 17 \\
           No. of Source Nodes of Type Session Storage & 0.0008 & 18 \\
           No. of Source Nodes of Type Script & 0.0006 & 23 \\
           No. of DOM Nodes Created By Scripts & 0.0005 & 25 \\
           No. of Edges of Type Remove Event Listener & 0.0004 & 26 \\
           No. of Edges of Type Add Event Listener & 0.0003 & 28 \\
           No. of Navigator Web API Calls & 0.0003 & 29 \\
           No. of Target Nodes of Type Script & 0.0003 & 31 \\
           No. of Screen Web API Calls & 0.0002 & 37 \\
           No. of Edges of Type Cross DOM & 0.0002 & 38 \\
           No. of Local Storage Read Storage Calls & 0.0001 & 39 \\
          \midrule
          Structural and Behavioral Features & \\
          \midrule
           No. of Source Nodes of Type Parser & 0.0022 & 7 \\
           No. of Edges of Type Create Node & 0.0017 & 12 \\
           No. of Edges of Type Insert Node & 0.0012 & 16 \\
           No. of HTML Elements Created & 0.0006 & 21 \\
           No. of Edges of Type Create Node & 0.0003 & 30 \\
           No. of Edges of Type Delete Attribute & 0.0002 & 34 \\
          \midrule
          Network Features & \\
          \midrule
          Sum of Bytes Transferred by Requests & 0.0083 & 1 \\
          Sum of Bytes Transferred by Requests & 0.0055 & 2 \\
          No. of Resources Blocked & 0.0006 & 24 \\
          No. of Edges of Type Request Complete & 0.0003 & 27 \\
          No. of Resources Blocked & 0.0003 & 32 \\
      \end{tabular}
  \end{center}
  \caption{Feature importance TODO: Remove ``duplicates''}
%   \label{table:feature_importance}
\end{table}

==> unused-bits/old_classifier_construction_bits.tex <==
\begin{enumerate}
    \item \textbf{Feature Design}, i.e. XXX auto-generated vs. expert-curated
    \item \textbf{Intervention Point}, i.e. XXX pre-intervention page vs. effect of intervention
    \item \textbf{Absolute vs. Relative}, i.e. XXX absolute feature value counts vs. ratio between feature value counts of the effect of intervention and the pre-intervention page
    \item \textbf{Page Scope}, i.e. XXX full page vs. intervention related
\end{enumerate}
A total of \NumFeatures{} features are extracted, decomposing into \NumAutoGeneratedFeatures{} auto-generated features and \NumExpertFeatures{} expert features as summarised in table \ref{table:features}.


==> unused-bits/old_intro_bits.tex <==
The \Web{} privacy community has suggested a lot of ways to improve privacy by
modifying browsers.

These works are good at measurement the privacy \emph{benefits} they bring, but
lack a way to measure compatibility \emph{costs}.

This is important since tools that break a lot of sites are not useful to most
users, and so in practice not very privacy improving.

What compatibility measurements do exist are either broad and aggregate (and so
make it difficult to determine which sites are broken), or narrow and manual
(and so don't scale).

The lack of an automated, scalable way of measuring the compatibility
cost of a proposed privacy intervention causes real privacy harm: ambitious
and novel projects may not see real world adoption, and current projects
will be risk averse.

Automated compatibility detection is difficult: theres a huge range
of ways that a site can be broken (\EG{} missing page elements, interactivity
reduced or modified, form submission or validation missing). These
an equally large range of ways ``brokenness'' might appear to the user, ranging
from easy to detect (\EG{} the page is blank) to extremely subtle (\EG{}
an event listener not firing after several earlier user action).

This work tries to improve that by building a fully automated classifier that
can determine whether a privacy intervention (here, a filter
list rule) will break a website. Our classifier requires no human action
to run, and runs in a heavily-modified desktop \Web{} browsers, and so can
scale far beyond what is possible with human assessments. Our classifier
takes as input i) a filter list rule, and ii) a website URL, and returns a
prediction of whether executing the given website \emph{with the given
filter list rule applied} will break the website, in the subjective
determination of a human.

We build our classifier in two novel steps. First, we use the commit
history of the EasyList project to build up a labeled dataset of filter list
rules that did (and did not) break websites, in the subjective evaluation
of the users and maintainers of EasyList authors and users.

And second,
we use a heavily modified version of Chromium-based browser to analyze
the execution of the website. Significantly, our modified browser (built
from an existing system called PageGraph) records both what events occurred
during the website's execution (\EG{} which scripts were executed, which
DOM notes were inserted or modified, which event listeners were registered),
and which actors on the page were responsible for each event (\EG{}
which script fetched a given resource, or inserted a DOM element, or fetched
a dependent script). Our PageGraph-instrumented browser then allows us
to export the recording of each page execution as a XML-encoded graph.

We then combine these two sources of data to generate a large dataset of
website executions, where we know (or are highly confident) that the site
was working or broken, in the subjective determination of a browser user.
More specifically, we generate \NumDataPoints{}, each with a label of
\texttt{\{broken, working\} X \{``with rule applied'', ``without rule applied''\}}.
We then extract \NumFeatures{} features from each data point, and train
a classifier that performs with AUC of \ClassifierAUC{}.
